Centralized Cooperative Exploration Policy for Continuous Control Tasks

The deep reinforcement learning (DRL) algorithm works brilliantly on solving various complex control tasks. This phenomenal success can be partly attributed to DRL encouraging intelligent agents to sufficiently explore the environment and collect diverse experiences during the agent training process. Therefore, exploration plays a significant role in accessing an optimal policy for DRL. Despite recent works making great progress in continuous control tasks, exploration in these tasks has remained insufficiently investigated. To explicitly encourage exploration in continuous control tasks, we propose CCEP (Centralized Cooperative Exploration Policy), which utilizes underestimation and overestimation of value functions to maintain the capacity of exploration. CCEP first keeps two value functions initialized with different parameters, and generates diverse policies with multiple exploration styles from a pair of value functions. In addition, a centralized policy framework ensures that CCEP achieves message delivery between multiple policies, furthermore contributing to exploring the environment cooperatively. Extensive experimental results demonstrate that CCEP achieves higher exploration capacity. Empirical analysis shows diverse exploration styles in the learned policies by CCEP, reaping benefits in more exploration regions. And this exploration capacity of CCEP ensures it outperforms the current state-of-the-art methods across multiple continuous control tasks shown in experiments.

==> sections/Abstract.tex <==
\begin{abstract}

The deep reinforcement learning (DRL) algorithm works brilliantly on solving a wide variety of complex control tasks. This phenomenal success can be attributed to DRL encouraging intelligent agents to sufficiently explore the environment and collect massive experiences during the agent training process. Promoting exploration efficiency is a promising avenue in enhancing the DRL algorithm performance. 

In practice, whereas updating with the same experience during training, it is rather hard to obtain two value functions initialized with different random seeds that are the same. The gap between these two value functions is termed on \textit{controversy}, which sees a decreasing trend along with the value function updating process. Based on this evidence, we propose CCEP (\textbf{C}entralized \textbf{C}ooperative \textbf{E}xploration \textbf{P}olicy), \textit{which is the first cooperative exploration in DRL venues.} CCEP first approximates two value functions initialized with different parameters and generates diverse policies with multiple exploration styles from the controversy between value functions. Then, we propose a centralized framework to achieve message delivery between different policies, furthermore making the contributions to explore the environment cooperatively. Extensive experimental results demonstrate that our proposed method achieves higher exploration  efficiency and outperforms the performance of current state-of-the-art methods across multiple continuous control environments. Besides, additional analysis verifies there exists differences in styles of exploration between our learned policies causing a wider range of exploration region applying our CCEP algorithm.

\end{abstract}
\keywords{Deep Reinforcement Learning, Cooperative Exploration, Continuous
Control Tasks}

==> sections/intro_new.tex <==
\section{introduction}
Deep reinforcement learning (DRL)~\cite{sutton_reinforcement_2018}, which utilizes deep neural networks to learn an optimal policy, works brilliantly and has demonstrated beyond human-level performance on solving various challenging sequential decision-making tasks e.g., video games~\cite{mnih2015human,mnih2016asynchronous,chen2021wide,xu2022side,ZHANG2022341}, autonomous driving~\cite{Ye2019automated}, robotic control tasks~\cite{andrychowicz2017hindsight, lillicrap2015continuous}, etc. In DRL settings, an agent needs to sufficiently explore the environment and collect a set of experiences to obtain an optimal policy. Even though recent works have made great success in continuous control tasks, exploration in such settings has not been sufficiently well studied. In this paper, we tackle the exploration issue in continuous control tasks.

It is essential that during the training phase the agent should be encouraged to explore the environments and gather sufficient reward signals for well training.

In online RL, exploration has obsessed with a critical problem: submitting solutions too quickly without sufficient exploration, leading to get stuck at local minima or even complete failure. DRL researchers adapt the neural network to yield the policy with significant feature extraction and expression capabilities in a range of continuous control tasks. This phenomenal practice has achieved great performance, but it is still obsessed with the notorious insufficient exploration problem.
Good exploration becomes extremely difficult when the environment provides little feedback or is distracting.
Whereas existing exploration methods remain a problematic drawback -- lacking diversity to explore. The classic exploration methods such as $\epsilon$-Greedy strategies~\cite{mnih2015human} or Gaussian noise~\cite{lillicrap2015continuous} indirectly and implicitly change the style of the exploration. However, in massive situations, diverse styles of exploration is necessary. For instance, in chess games, players should perform different styles of policies (e.g., radical, conservative, etc.) to keep competitive when facing 
various situations; humanoid robots attempt diverse control styles and eventually learn to walk efficiently.

Recent studies enrich diverse styles of policies by constructing relationships between the distribution of policy and trajectories~\cite{achiam2018variational,florensa2017stochastic,sharma2019dynamics}. In Diversity is All You Need (DIAYN)~\cite{eysenbach2018diversity}, authors highlight the diversity of policies plays a significant role in well-training agents. It trains the policy that maximizes the mutual information between the latent variable and the states, then altering the latent variable of the policy network creates multiple policies performing disparately. Although this interested viewpoint has attracted a spectrum of following works~\cite{achiam2018variational,eysenbach2018diversity,florensa2017stochastic,gregor2016variational,sharma2019dynamics}, aforementioned methods achieve diverse policies depending on the task in an unsupervised way, resulting in the algorithm performing insufficient generality in different tasks. In fact, the ideal algorithm to implement the diverse policies should be general across a range of tasks, which motives us to design \textit{task-oriented} algorithm working towards developing various policies. Eysenbach et al. proposed~\citep{eysenbach2021information} that the learned skills could not construct all the state marginal distributions in the downstream tasks. For task relevance, the mutual information is added as an intrinsic reward for empowerment~\cite{mohamed2015variational,choi2021variational}, but these methods change the original reward function resulting in the performance being extremely sensitive to the trade-off between original and intrinsic rewards.

Our method insights from a interesting phenomenon during the exploration. The critic aims to approximate the accumulated reward by bootstrapping in the actor-critic framework. However, the different critic functions may have great differences even if they approximate the same target due to the function approximation error. For instance, Twin Delayed Deep Deterministic policy gradient (TD3)~\cite{fujimoto2018addressing} presents that two value functions with different initial parameters perform quite differently with the identical targets. It is knotty to measure whether a value function is exact or not, and the gap between these two value functions is termed on \textit{controversy}, which sees a decreasing trend along with the value function updating process. Our intuition can be ascribed that controversy in the value estimation will lead to sub-optimal policies, and these policies have a bias toward message acquisition known as the \texttt{style}.

This paper highlights that controversy can be utilized to encourage policies to yield multiple styles, and encourages exploration for a continuous control task by applying multi-styled policies. Our paper contributes three aspects. (1) We first describe that the estimation bias in double value functions can lead to various exploration \texttt{styles}. (2) This paper proposes the CCEP algorithm, encouraging diverse exploration for environments by cooperation from multi-styled policies. (3) Finally, in CCEP, we design a novel framework, termed as centralized value function framework, which is updated by experience collected from all the policies and accomplishes the message delivery mechanism between different policies.  
Extensive experiments are conducted on the MuJoCo platform to evaluate the effectiveness of our method. The results reveal that the proposed CCEP approach attains substantial improvements in both average return and sample efficiency on the baseline across selected environments, and the average return of agents trained using CCEP is $6.7\%$ higher than that of the baseline. Besides, CCEP also allows agents to explore more states during the same training time steps as the baseline. Additional analysis indicates that message delivery leading to the cooperative multi-styled policies further enhances the exploration efficiency $8.6\%$ compared with that of without cooperation.


We organize the rest of this paper as follows. Section~\ref{sec:related} discusses related works. Then, Section~\ref{sec:preliminaries} briefly explains the concepts of RL. We elaborate on how to perform the CCEP algorithm in Section~\ref{sec:CCEP}. We introduce our experimental settings in Section~\ref{sec:setup}. Section~\ref{sec:result} presents and analyzes results to validate the effectiveness of CCEP, after which we conclude our paper in Section~\ref{sec:conclusion}. The code and documentation are released in the anonymous link for validating reproducibility.\footnote{\label{link:open}\url{https://anonymous.4open.science/r/CCEP-67F1}}
%\gc{This paper highlights that controversy can be utilized to encourage policies to yield multiple styles. Our paper contributes to constructing controversy from three aspects.} The first contribution describes the difference between the two value functions with the same target and the training process, revealing the degree of positive bias as TD3 use these differences to reduce overestimation. \gc{Second, we initialize the value functions $Q_1$ and $Q_2$ (also known as \texttt{critic} network in actor-critic framework) with two separate sets of random parameters. These} two critic networks have a controversy on value estimations because of their styles. To increase the difference in the distribution, the two value functions were given a pair of opposite targets. This would guarantee the difference between the distribution of the value functions even if the two value functions were set to the same parameters as the initial. Experimental results presented in this paper show how much will these two value functions affect the policy.
%Third, to encourage diverse styles, there are two other critics. One of them is a radical critic and always gives a high value $max(Q_1, Q_2)$, and the other is a conservative critic and always gives less value $min(Q_1, Q_2)$. With these critics, our proposed algorithm trains policies with diverse styles to encourage centralized cooperative exploration. We present two key technical contributions that make this a practical exploration method. First, we feed latent variables and one-hot labels as a distinguishing input to the policy to represent different styles. These policies optimize unique critics separately. The intuition is that the two value functions with the same target converge into the same value distribution along with the training process so as the minimum or the maximum of them. However, the maximum of the two value functions makes the policy concentrate more on the higher value of a state and vice versa. The different concentration makes the different style of policy. Second, we randomly sample the latent variable $z$ at each time step so that the exploration process is done cooperatively. 


